Don't Read Too Much into It: Adaptive Computation for Open-Domain Question Answering

Most approaches to Open-Domain Question Answering consist of a light-weight retriever that selects a set of candidate passages, and a computationally expensive reader that examines the passages to identify the correct answer. Previous works have shown that as the number of retrieved passages increases, so does the performance of the reader. However, they assume all retrieved passages are of equal importance and allocate the same amount of computation to them, leading to a substantial increase in computational cost. To reduce this cost, we propose the use of adaptive computation to control the computational budget allocated for the passages to be read. We first introduce a technique operating on individual passages in isolation which relies on anytime prediction and a per-layer estimation of an early exit probability. We then introduce SkylineBuilder, an approach for dynamically deciding on which passage to allocate computation at each step, based on a resource allocation policy trained via reinforcement learning. Our results on SQuAD-Open show that adaptive computation with global prioritisation improves over several strong static and adaptive methods, leading to a 4.3x reduction in computation while retaining 95% performance of the full model.

==> Adaptive Computation Open Domain QA/abstract-odqa.tex <==
Most approaches to \acrlong{ODQA} consist of a light-weight retriever that selects a set of candidate passages,
and a computationally expensive reader that examines the passages to identify the correct answer.
%
%
Previous works have shown that as the number of retrieved passages increases, so does the performance of the reader.
%
%
%
%
%
%
%
%
%
%
%
%
However, they assume all retrieved passages are of equal importance and allocate the same amount of computation to them, leading to a substantial increase in computational cost.
%
To reduce this cost, we propose the use of \emph{adaptive computation} to control the computational budget allocated for the passages to be read. 
%
%
We first introduce %ADAPATIVE-ISOLATED-ODQA
%
a technique operating on individual passages in isolation which relies on anytime prediction and a per-layer estimation of an early exit probability. %the early exit probability, stopping computation when this probability exceeds a threshold. 
%
We then introduce \globalmethodRL{}, an approach %that globally assesses all passages in terms of where to allocate computation to next and uses Reinforcement Learning to optimise its resource allocation strategy.
for dynamically deciding on which passage to allocate computation at each step, based on a resource allocation policy trained via reinforcement learning.
%
Our results on SQuAD-Open show that adaptive computation with global prioritisation improves over several strong static and adaptive methods, leading to a 4.3x reduction in computation while retaining 95\% performance of the full model.  
%


==> Adaptive Computation Open Domain QA/adaptive_odqa.tex <==
%
%
%
%
%

\section{Background}

\newcommand{\layer}{\ensuremath{\mathrm{TransformerLayer}}}
\newcommand{\outputlayer}{\ensuremath{\mathrm{OutputLayer}}}
\newcommand{\logitslayer}{\ensuremath{\mathrm{Logits}}}
\newcommand{\softmax}{\ensuremath{\mathrm{Softmax}}}
\newcommand{\sigmoid}{\ensuremath{\mathrm{Sigmoid}}}
\newcommand{\mlp}{\ensuremath{\mathrm{MLP}}}

\newcommand{\problayer}{\ensuremath{\mathrm{P}_{\text{out}}}}
\newcommand{\logits}{\ensuremath{\mathbf{s}}}
\newcommand{\x}{\ensuremath{\mathbf{x}}}
\newcommand{\threshold}{\ensuremath{\tau}}
\newcommand{\noanswer}{\ensuremath{\mathrm{NoAnswer}}}
\newcommand{\hasanswer}{\ensuremath{\mathrm{HasAnswer}}}

\newcommand{\hidden}{\ensuremath{\mathbf{a}}}
\newcommand{\hiddent}{\ensuremath{\mathbf{h}}}

\newcommand{\result}{\ensuremath{\mathbf{y}}}
\newcommand{\query}{\ensuremath{\mathbf{q}}}
\newcommand{\corpus}{\ensuremath{C}}
\newcommand{\docset}{\ensuremath{D}}
\newcommand{\reader}{\ensuremath{\mathrm{Reader}}}
\newcommand{\passagereader}{\ensuremath{\mathrm{PReader}}}
\newcommand{\aggregate}{\ensuremath{\mathrm{Agg}}}
\newcommand{\CLS}{\ensuremath{\mathrm{CLS}}}
\newcommand{\currepr}{\ensuremath{A}}
\newcommand{\curheight}{\ensuremath{H}}
\newcommand{\state}{\ensuremath{S}}
\newcommand{\height}{\ensuremath{h}}
\newcommand{\buildupphase}{\ensuremath{\mathrm{BuildUp}}}
\newcommand{\outputphase}{\ensuremath{\mathrm{Output}}}

\newcommand{\numoutputs}{\ensuremath{m}}
\newcommand{\priority}{\ensuremath{p}}
\newcommand{\heightembed}{\ensuremath{\mathrm{HeightEmb}}}
\newcommand{\rankembed}{\ensuremath{\mathrm{IndexEmb}}}
\newcommand{\action}{\ensuremath{\mathbf{i}}}
\newcommand{\prioritymodel}{\ensuremath{\mathrm{PriorityModel}}}
\newcommand{\alllayer}{\ensuremath{\mathrm{AnyLayer}}}
\newcommand{\lastlayer}{\ensuremath{\mathrm{LastLayer}}}

\newcommand{\devzero}{\ensuremath{\mathrm{dev_{0}}}}
\newcommand{\devone}{\ensuremath{\mathrm{dev_{1}}}}

\newcommand{\numpassages}{\ensuremath{n}}  % number of passages
\newcommand{\budget}{\ensuremath{b}}  % number of passages



%
%
%
%
%
%
%
%
%
%
%
%
We first give an overview of \acrshort{ODQA} and the relevant work in adaptive computation. 

\subsection{Open Domain Question Answering}
%
In \acrshort{ODQA} we are given a natural language query $\query$ and a large number of passages $\corpus$---for example, all paragraphs in Wikipedia. The goal is to use $\corpus$ to produce the answer \result{}.
%
In extractive \acrshort{ODQA} this answer corresponds to a span in one of the documents of $\corpus$.
%
%
%
%
%
The corpus \corpus{} can be very large, and a common approach to reduce computational costs is to first determine a smaller document set $\docset_{\query} \subseteq \corpus$ by retrieving the most relevant $\numpassages{}$ passages using an information retrieval module. Then we run a neural reader model on this subset.
%
%
%
In most works, the reader model extracts answers by applying a per-passage reader to each input passage $\x_{1}, \ldots, \x_{\numpassages{}} \in \docset_{\query}$ and then apply some form of aggregation function on the per-passage answers to produce a final answer.  %$\aggregate(\passagereader(\query,\x_{1}),\ldots,\passagereader(\query,\x_{\numpassages{}}))$.
%
Note that the passage reader can either produce an answer span as output, or %return 
$\noanswer$ in case the passage does not contain an answer for the given question. 

%
\subsection{Transformers for ODQA}
%
%
Most current \acrshort{ODQA} models rely on transformer-based architectures~\citep{DBLP:conf/nips/VaswaniSPUJGKP17}, usually pre-trained, to implement the \passagereader{} passage reader interface.
%
%
%
In such models, an input passage is processed via a sequence of transformer layers; in the following, we denote the $i$-th transformer layer in the sequence as $\layer_i$.
%
%
%
%
Let $\hiddent_i$ be the input to the $i$-th transformer layer and $\hiddent_{i+1} = \layer_i(\hiddent_i)$ its output. We set $\hiddent_1 = \x$ to be the input passage.
%
In standard non-adaptive Transformer-based models, we incrementally build a \emph{tower}---a composition of Transformer layers---until we reach some pre-defined height $n$ and use an output layer to produces the final output,  $\result=\outputlayer(\hiddent_n)$.
%
%
%
%
In this work, due to efficiency reasons, we restrict ourselves to pre-trained ALBERT~\citep{DBLP:conf/iclr/LanCGGSS20} models. One critical property of these models is parameter tying across layers: $\layer_i(\hiddent)=\layer_j(\hiddent)$ for any $i,j$.
%

\subsection{Adaptive Computation}
Our goal is to early-exit the iterative layer-by-layer process in order to save computation.
%
We assume this can be happening adaptively, based on the input, since some passages might require less computation to produce an answer than others.
%
\citet{DBLP:conf/acl/SchwartzSSDS20} show how this can be achieved for classification tasks. They first require internal layers to be able to produce outputs too, yielding an \emph{anytime} algorithm.~\footnote{In practice, \citet{DBLP:conf/acl/SchwartzSSDS20} choose a subset of layers to be candidate output layers, so strictly speaking we cannot exit any time, but only when a candidate layer is reached.} This can be achieved with a suitable training objective. Next, for each candidate layer $i$, they calculate the %output layer 
exit probability given its hidden state $\hiddent_i$, and use them for taking an early-exit decision: if the highest exit probability is above a global threshold $\threshold$, they return $\outputlayer(\hiddent_i)$ otherwise they continue with the following layers.
%

%
The output layer probabilities %by themselves 
are not %optimally 
calibrated for exit decisions, and hence \citet{DBLP:conf/acl/SchwartzSSDS20} tune them on an held-out validation set via temperature calibration~\citep{DBLP:conf/icml/GuoPSW17,DBLP:journals/corr/abs-2003-07892}, where a temperature $T$ is tuned to adapt the softmax output probabilities at each layer. 
%
%
%
%
%


==> Adaptive Computation Open Domain QA/experiments.tex <==
\paragraph{Dataset}
%
%
%
SQuAD-Open~\citep{DBLP:conf/acl/ChenFWB17} is a popular open-domain question answering dataset based on SQuAD. %and a popular \acrshort{ODQA} benchmark. 
We partition the dataset into four subsets: training set, two development sets (\devzero{} and \devone{}), and test set, and their details are summarised in \cref{tab:datasize}. %. The need for two development sets is described below, and the dataset sizes are shown in \cref{tab:datasize}.

\begin{table}[t]
%
\resizebox{\columnwidth}{!}{
    \begin{tabular}{lcccc}
      \toprule
      {\bf SQuAD-Open} & { train} \ & { \devzero{} } \ & { \devone{} } \ & { test} \\
      \midrule
      Size & 78,839 & 4,379 & 4,379 & 10,570  \\
      Hits@30 & 71.2\% & 72.7\% & 72.1\% & 77.9\% \\
      \bottomrule
    \end{tabular}
}
\caption{Dataset sizes and retriever performances.} \label{tab:datasize}
%
\end{table}


\paragraph{Experimental Setup}

We follow the preprocessing approached proposed by \citet{DBLP:conf/emnlp/WangNMNX19} and split passages into 100-word long chunks with 50-word long strides. We use a BM25 retriever 
%
to retrieve the top $\numpassages$ passages for each question as inputs to the reader and the Wikipedia dump provided by \citet{DBLP:conf/acl/ChenFWB17} as source corpus.  Following \citet{DBLP:conf/emnlp/WangNMNX19}, we set $\numpassages=5$ for training and  $\numpassages = 30$ for test evaluations.
%
\cref{tab:datasize} shows the Hits@30 %performance 
results of our BM25 retriever on the dataset and they are comparable with previous works~\citep{DBLP:conf/naacl/YangXLLTXLL19,DBLP:conf/emnlp/WangNMNX19}.
%


\paragraph{Reader Model}
%
For all our experiments, we fine-tune a pre-trained ALBERT model~\citep{DBLP:conf/iclr/LanCGGSS20}, consisting of 24 transformer layers and cross-layer parameter sharing.
%
%
%
We do \emph{not} use global normalisation~\citep{DBLP:conf/acl/GardnerC18} in our implementation, but our full system (without adaptive computation) achieves an EM score of 52.6 and is comparable to Multi-passage BERT~\citep{DBLP:conf/emnlp/WangNMNX19} which uses global normalisation.




\paragraph{Training Pipeline}
%
%
The anytime reader models are first trained on training set and validated on \devzero{}. Then we conduct temperature calibration on \devzero{}. 
For \globalmethodRL{}, the scheduler model is trained on \devzero{} with the calibrated anytime model, and validated with \devone{}.
%
%
%


\paragraph{Baselines}
Following \citet{DBLP:conf/acl/SchwartzSSDS20}, we use three types of baselines: 
\begin{inparaenum}[\itshape 1\upshape)]
    \item the \emph{standard baseline} that reads all passages and outputs predictions at the final layer,
    \item the \emph{efficient baseline} that always exits at a given intermediate layer for all passages, and is optimised to do so, 
    \item the \emph{top-$k$ baseline} that only reads the $k$ top ranked passages and predicts the answer at their final layers.
\end{inparaenum}



\begin{figure*}[t]
\begin{center}
\begin{subfigure}{.49\textwidth}
\includegraphics[width=\textwidth]{figures/em_squad_test_master.pdf}
\subcaption{\globalmethodRL{} vs. baselines} \label{fig:master}
\end{subfigure}
%
\begin{subfigure}{.49\textwidth}
\includegraphics[width=\textwidth]{figures/em_squad_test_local_vs_global.pdf}
\subcaption{Local vs. Global Models} \label{fig:local_vs_global}
\end{subfigure}
%
\begin{subfigure}{.49\textwidth}
\includegraphics[width=\textwidth]{figures/em_squad_test_anytime_vs_lastlayer.pdf}
\subcaption{\alllayer{} vs. \lastlayer{}} \label{fig:anytime_vs_lastlayer}
\end{subfigure}
%
\begin{subfigure}{.49\textwidth}
\includegraphics[width=\textwidth]{figures/em_squad_test_init_priority.pdf}
\subcaption{Learnt vs. Fixed Initial Priorities} \label{fig:init_priority}
\end{subfigure}
%
\end{center}
\caption{Evaluation results on the SQuAD-Open test set with 30 passages.} \label{fig:results}
\end{figure*}


\paragraph{Evaluation protocol}
Our goal is to assess the computational efficiency of a given method in terms of accuracy vs. computational budget used. 
%
%
%
We follow \citet{DBLP:conf/iclr/FanGJ20} and consider the computation of one layer as a unit of computational cost. In particular, we will assess how many layers, on average, each method builds up for each passage. 
%
%
%
%
Similarly to \citet{DBLP:conf/acl/SchwartzSSDS20}, we show the accuracy-efficiency trade-off for different strategies by showing the computation cost on the $x$-axis, and the Exact Match (EM)~\footnote{The evaluation script can be found at this address: \href{https://github.com/facebookresearch/DrQA}{https://github.com/facebookresearch/DrQA}.} score on the $y$-axis.
%
%
%

%
%
%

%
%
%
%
\subsection{Static vs. Adaptive Computation}
%
We first investigate how adaptive computation compares to the static baselines. We will focus on a single adaptive method, \globalmethodRL{}, and assess different adaptive variants later. 

\cref{fig:master} shows the accuracy of \globalmethodRL{} at different budgets when compared to the standard, efficient, and top-$k$ baselines. 
We note that it reaches the similar results of the static baselines with much fewer layers.
In particular, it yields substantially higher performance than static methods when the computational budget is smaller than ten layers. For example, when given four layers on average, \globalmethodRL{} achieves EM score 48.0, significantly outperforming EM score 44.2 of the top-$k$ baseline.
%

%
In \cref{tab:budget_em} we consider a setting where \globalmethodRL{} and the static baseline reach comparable (95\%) performance of the full 24-layer model.
%
We see that simply reducing the number of passages to process is giving a poor accuracy-efficiency trade-off, requiring 14.4 layers (or 18 passages) to achieve this accuracy. %for this level of exact match accuracy.
%
The efficient baseline fares better with 9.5 layers, but it is still outperformed by \globalmethodRL{}, that only needs 5.6 layers on average to reach the desired accuracy.
%




\begin{table}[t]
%
\resizebox{\columnwidth}{!}{
    \begin{tabular}{lcc}
      \toprule
      {\bf Method} & {\bf Avg. \#layers} \ & {\bf Reduction } \  \\
      \midrule
      Standard baseline & 24 & 1.0x  \\
      Efficient baseline & 9.5 & 2.5x  \\
      Top-$k$ baseline & 14.4 & 1.7x  \\
      \midrule
      \localmethod{} & 9.0 & 2.7x  \\
      \globalmethod{} & 6.1 & 3.9x  \\
      \globalmethodRL{} & \bf{5.6} & \bf{4.3x}  \\
      \bottomrule
    \end{tabular}
}
\caption{Reduction in layer computations while achieving 95\% of the accuracy of the standard baseline.} \label{tab:budget_em}
%
\end{table}

%
%
%
%
%


\begin{table*}[!hbt]
%
%
\begin{center}
\resizebox{\textwidth}{!}{
\begin{tabular}{lcccccc}
  \toprule
   & { $\text{Var}(h)$} \ & { $\text{Avg}(\text{rank})$ } \ & { Flips} \ & { $h_{+}-h_{-}$} \ & { HAP} \ & { Exact Match} \\
  \midrule
  Efficient Baselines & 0.00 & 14.50 & - & 0.00 & 6.1\% & 23.47 \\
  \midrule
  \localmethod{} & 11.05 & 13.38 & - & 3.68 & 22.0\% & 17.10 \\
  \midrule
  \globalmethod{} & 7.46 & 13.06 & 13.37 & 3.46 & 27.4\% & 27.95 \\
  \globalmethodRL{} & 12.71 & 8.78 & 6.48 & 5.99 & {40.5}\% & {\bf 33.60} \\
  \bottomrule
\end{tabular}
}
\caption{Quantitative analysis on SQuAD Open \devone{} set with top 30 passages and two layers of computation per passage on average.} \label{tab:analysis}
\end{center}
%
\end{table*}




%
%
\subsection{Local vs. Global Models} \label{ssec:glocal}
What is the impact of globally selecting which towers to extend, rather than taking early-exit decisions on a per-tower basis? %in a global level as opposed to per-tower processing with exit probabilities?
%
To answer this question, we consider two global methods: \globalmethodRL{} and \globalmethod{}, %, \globalmethod{}(without RL)
the method in \cref{ssec:global} that uses $\hasanswer$ probabilities as priorities without any RL-based selection policy.
We compare both to the local method \localmethod{}. %and focus on computation budgets up to 12 layers, since we observe that after this threshold all methods perform similarly.
%

\cref{fig:local_vs_global} shows that, while for very low budgets \localmethod{} outperforms \globalmethod{}, with a budget larger than 4 layers it is not the case anymore.
%
This may be due to a tendency of \globalmethod{} spending an initial computation budget on exploring many towers---in \cref{fig:tower_vis} we show examples of this behaviour.
%
It is also shown that \globalmethodRL{} considerably outperforms both \localmethod{} and \globalmethod{}.
%
%
%
%
%
Along with the results in \cref{tab:budget_em}, the comparisons above indicate that 
\begin{inparaenum}[\itshape 1\upshape)]
    \item global scheduling across multiple towers is crucial for improving efficiency, and
    \item optimising the adaptive policy with RL manage to exploit global features for tower selection, leading to further improvements.
\end{inparaenum}



\subsection{Ablation Studies}
%
\paragraph{Any Layer vs. Last Layer Model} \label{sec:alllayer_vs_lastlayer}
%
%
For comparing the $\lastlayer$ and the $\alllayer$ strategies introduced in \cref{ssec:local}, we show the behaviour of these methods for the \globalmethodRL{} scheduling algorithm in \cref{fig:anytime_vs_lastlayer}.
%
Using an anytime answer extraction model has a negative effect on accuracy. We see this clearly at 24 layers where $\alllayer$ lags substantially behind the standard baseline while $\lastlayer$  almost reaches it. 
We see this gap across the whole budget spectrum, leading to less accurate results except for very small budgets.
%
%
%
%

%
%
%
%
%
%
%
%
\paragraph{Learning Initial Priorities}
\globalmethodRL{} uses a learnt initial priority for each tower. This not only enables it learn which towers to process first at the beginning, but also how long to wait until other towers are visited. 
%
\cref{fig:init_priority} shows the benefit gained from adopting this strategy: without training the initialisation priorities, \globalmethodRL{} spend more computation on passages that are likely not needed.
%
Once an average of 4 layers have been added, the benefit disappears as \globalmethodRL{} with learnt initial priorities will try to visit more candidates itself.  
%
%
%
%
%



 
%
\subsection{Quantitative Analysis}
%
This section aims at understanding where and how our adaptive strategies behave differently, and what contributes to the gain in the accuracy-efficiency trade-off.
%
We propose the following quantitative metrics:
\begin{inparaenum}[\itshape 1\upshape)]
%
    \item $\text{Var}(h)$: variance of the heights of the towers. %This metric partly indicates how adaptive the method is.
    \item $\text{Avg}(\text{rank})$: average rank of the tower when the method chooses which tower to build on.
    \item Flips: how often does the strategy switch between towers, measuring the exploration-exploitation trade-off of a method. %. This measures how focused the method is.
    \item $h_{+}-h_{-}$: $h_{+}$ (resp. $h_{-}$) is the average height of towers with (resp. without) an answer. Their difference measures the difference in amount of computation between passages with the answer and the ones without an answer.
    \item \hasanswer{} Precision (HAP): how often a tower selection action selects a tower whose passage contains the answer.
%
\end{inparaenum}
%
%
%

%
We analyse our proposed methods along with static baselines on the SQuAD development set; results are outlined in \cref{tab:analysis}.
%
%
%
Overall, the higher the $\hasanswer$ Precision, the more accurate the method.
%
This finding matches with our intuition that, if a tower selection strategy can focus its computation on passages that contain the answer, it yields more accurate results with smaller computation budgets. %a better performances with a lower budget.

Comparing \globalmethod{} and \globalmethodRL{} gives more insights regarding what the RL training scheme learns.
%
\globalmethodRL{} learns a policy with the highest $\text{Var}(h)$, the lowest $\text{Avg}(\text{rank})$, and the lowest number of tower flips, suggesting that 
\begin{inparaenum}[\itshape 1\upshape)]
    \item it focuses on a few towers rather than distributing its computation over all passages,
    \item it is more likely to select top-ranked passages, and 
    \item it switches less between towers, and tends to build one tower before switching to another.
\end{inparaenum}
%
\globalmethodRL{} also yields the highest $\hasanswer$ Precision and $h_{+}-h_{-}$, meaning that tends to prioritise the passages containing the answer. %positive passages over negative ones.


\begin{figure}[!tb]
\begin{center}
\begin{subfigure}{\columnwidth}
\begin{center}
\fbox{\includesvg[height=3.2cm]{figures/visualise/towers/skylinebuilder_39.svg}}
\fbox{\includesvg[height=3.2cm]{figures/visualise/towers/skylinebuilderRL_39.svg}}
\end{center}
\subcaption{Example 1} \label{ex:1}
\end{subfigure}
%
%
\begin{subfigure}{\columnwidth}
\begin{center}
\fbox{\includesvg[height=3.2cm]{figures/visualise/towers/skylinebuilder_1231.svg}}
\fbox{\includesvg[height=3.2cm]{figures/visualise/towers/skylinebuilderRL_1231.svg}}
\end{center}
\subcaption{Example 2} \label{ex:2}
\end{subfigure}
%
\begin{subfigure}{\columnwidth}
\begin{center}
\fbox{\includesvg[height=3.2cm]{figures/visualise/towers/skylinebuilder_117.svg}}
\fbox{\includesvg[height=3.2cm]{figures/visualise/towers/skylinebuilderRL_117.svg}}
\end{center}
\subcaption{Example 3} \label{ex:3}
\end{subfigure}
%
\end{center}
\caption{Examples of the skylines built by \globalmethod{} (left) and \globalmethodRL{} (right), with two layers per passage on average. %The towers are ordered by the rank of the passages from left to right and are built from bottom to top.
The green blocks indicate towers that contain the answer. %and the colour gradient of the blues blocks reflects the order in which the layers are built, the darker the later.
%
} \label{fig:tower_vis}
\end{figure}
  
  
 

\subsection{Qualitative Analysis and Visualisation}
%
%
%
%
Here we analyse how different methods build the skyline.
%
\cref{fig:tower_vis} shows some examples of skylines built by \globalmethod{} and \globalmethodRL{}. %with budget $\budget_{\numpassages=30}$. 
The towers are ordered by the rank of their associated passages in the retrieval results from left to right, and are built bottom-up. %from bottom to top.
%
The colour gradient of the blues blocks reflects the order in which the layers are built: darker cells correspond to layers created later in the process. %the darker the later.

In \cref{ex:1} and \cref{ex:2} we can see that \globalmethodRL{} tends to focus on one or two towers,
whereas \globalmethod{} %scatter its layers over towers
has a more even distribution of computation across different towers.
%
%
%
In \cref{ex:2}, even when only one tower contains the answer, \globalmethodRL{} manages to locate it and build a full-height tower on it.

\cref{ex:3} shows a case where none of the top 4 passages contains the answer. \globalmethodRL{} goes over these irrelevant towers quickly and start exploring later towers, until it reaches the tower with rank 27 and becomes confident enough to keep building on it.
%
These examples shows how \globalmethodRL{} learns an efficient scheduling algorithm to locate passages containing the answer with very limited budgets.
%
%
%
%

\begin{figure}[t]
\begin{center}
\begin{subfigure}{\columnwidth}
\begin{center}
\fbox{\includesvg[height=3.2cm]{figures/visualise/heatmaps/skylinebuilder_heatmap.svg}}
\fbox{\includesvg[height=3.2cm]{figures/visualise/heatmaps/skylinebuilderRL_heatmap.svg}}
\end{center}
%
\end{subfigure}
\end{center}
\caption{Heatmap of the tower selections by \globalmethod{} (left) and \globalmethodRL{} (right). The colour gradient of the blues blocks reflects their selection frequencies.%, the darker the more frequent.
} \label{fig:heatmap}
\end{figure}

%
%
%
%
To understand how our proposed methods work at macro level, we use heat-maps (\cref{fig:heatmap}) for showing how frequently each block is selected.
%
The green row at the bottom indicates the frequency of each passage containing the answer.
%
\globalmethod{} explores all passages quite evenly, whereas \globalmethodRL{} learns to prioritise top-ranked towers. This preference is reasonable because, as shown by the green row at the bottom, top-ranked towers are more likely to contain the answer. 
%
Also note that \globalmethodRL{} does not naively process towers from left to right like the top-$k$ baseline does, but instead it learns a trade-off between \emph{exploration and exploitation}, leading to the significant improvement over the top-$k$ baseline shown in \cref{fig:master}.




\subsection{Adaptive Computation vs. Distillation} \label{sec:compare_distil}

Distillation is another orthogonal approach to reduce computational cost. We compare our adaptive computation method \globalmethodRL{} with a static DistilBERT~\citep{DBLP:journals/corr/abs-1910-01108} baseline, and the results are shown in \cref{tab:distilbert}. Our method significantly outperforms DistilBERT while computing much fewer layers. 

\begin{table}[t]
%
\resizebox{\columnwidth}{!}{
    \begin{tabular}{lcc}
      \toprule
      {\bf Models} & {\bf Num. layers} & {\bf EM} \\
      \midrule
      DistilBERT~\citep{DBLP:journals/corr/abs-1910-01108} & 6 & 40.5 \\
      \globalmethodRL{} & 1.6 & 41.1 \\
      \globalmethodRL{} & 3 & 46.4 \\
      \globalmethodRL{} & 6 & {\bf 49.7} \\
      \bottomrule
    \end{tabular}
}
\caption{Comparing adaptive computation with distillation on SQuAD-Open test set.} \label{tab:distilbert}
%
\end{table}


==> Adaptive Computation Open Domain QA/related.tex <==

\section{Related Work}
%
%
%
%
%
%
%
%
%
%
%
%
%
%

\paragraph{Adaptive Computation}
%
One strategy to reduce a model's complexity %at inference time 
consists in dynamically deciding which layers to execute during inference~\citep{DBLP:journals/corr/BengioBPP15,DBLP:journals/corr/Graves16}. %, where a recurrent model learns how many computational steps to take between receiving an input and emitting an output.
%
%
%
%
%
%
%
%
%
%
%
%
%
%
\emph{Universal transformers}~\citep{DBLP:conf/iclr/DehghaniGVUK19} %are a Transformer variant %with cross-layer parameter sharing  that 
can learn after how many layers to emit an output conditioned on the input.
%
\citet{DBLP:conf/iclr/ElbayadGGA20} generalise universal transformers by also learning which layer to execute at each step. %, whilst \citet{DBLP:journals/corr/abs-2002-08614} explore adaptive computation time both at encoding and decoding step in neural machine translation tasks.
%
%
%
%
%
\citet{DBLP:conf/acl/SchwartzSSDS20,DBLP:conf/acl/LiuZWZDJ20} propose methods that can adaptively decide when to early stop the computation in sentence classification tasks.
%
To the best of our knowledge, previous work has focused adaptive computation for a single input. We are the first to learn how to prioritise computation across instances %, and the first who look at this problem 
in the context of \acrshort{ODQA}. 

%
%
%
%
%



%
\paragraph{Smaller Networks}
Another strategy % for improving the efficiency during inference 
consists in training smaller and more efficient models.
%
In \emph{layer-wise dropout}~\citep{DBLP:conf/emnlp/LiuRSG0018}, during training, layers are randomly removed, making the model robust to layer removal operations.
%
This idea was expanded \citet{DBLP:conf/iclr/FanGJ20} to modern Transformer-based models.
%
%
%
Other methods include \emph{Distillation}~\citep{DBLP:journals/corr/HintonVD15} of a teacher model into a student model, \emph{Pruning} of architectures after training~\citep{DBLP:conf/nips/CunDS89} and \emph{Quantisation} of the parameter space~\citep{DBLP:journals/corr/abs-1805-10796,DBLP:journals/corr/abs-1909-05840,DBLP:journals/corr/abs-1910-06188}. 
%
%
%
%
%
%
%
%
%
%
%
%
%
%
These methods are not adaptive, but could be used in concert with the methods proposed here.
%
%

%


%
\paragraph{Open Domain Question Answering}
%
%
%
%
%
Most modern \acrshort{ODQA} systems adopt a two-stage approach that consists of a retriever and a reader, such as DrQA~\citep{DBLP:conf/acl/ChenFWB17}, HardEM~\citep{DBLP:conf/emnlp/MinCHZ19},  BERTserini~\citep{DBLP:conf/naacl/YangXLLTXLL19}, Multi-passage BERT~\citep{DBLP:conf/emnlp/WangNMNX19}, and PathRetriever~\citep{DBLP:conf/iclr/AsaiHHSX20}.
    %
%
%
%
%
%
%
%
%
%
As observed by \citet{DBLP:conf/acl/ChenFWB17,DBLP:conf/naacl/YangXLLTXLL19,DBLP:journals/corr/abs-2004-04906,DBLP:conf/emnlp/WangNMNX19}, the accuracy of such two-stage models increases with more passages retrieved.
%
%
But it remains a challenge to efficiently read a large number of passages as the reader models are usually quite computationally costly.
%

